Inapproximability of Matrix $p\rightarrow q$ Norms

We study the problem of computing the $p\rightarrow q$ norm of a matrix $A \in R^{m \times n}$, defined as \[ \|A\|_{p\rightarrow q} ~:=~ \max_{x \,\in\, R^n \setminus \{0\}} \frac{\|Ax\|_q}{\|x\|_p} \] This problem generalizes the spectral norm of a matrix ($p=q=2$) and the Grothendieck problem ($p=\infty$, $q=1$), and has been widely studied in various regimes. When $p \geq q$, the problem exhibits a dichotomy: constant factor approximation algorithms are known if $2 \in [q,p]$, and the problem is hard to approximate within almost polynomial factors when $2 \notin [q,p]$. The regime when $p < q$, known as \emph{hypercontractive norms}, is particularly significant for various applications but much less well understood. The case with $p = 2$ and $q > 2$ was studied by [Barak et al, STOC'12] who gave sub-exponential algorithms for a promise version of the problem (which captures small-set expansion) and also proved hardness of approximation results based on the Exponential Time Hypothesis. However, no NP-hardness of approximation is known for these problems for any $p < q$. We study the hardness of approximating matrix norms in both the above cases and prove the following results: - We show that for any $1< p < q < \infty$ with $2 \notin [p,q]$, $\|A\|_{p\rightarrow q}$ is hard to approximate within $2^{O(\log^{1-\epsilon}\!n)}$ assuming $NP \not\subseteq BPTIME(2^{\log^{O(1)}\!n})$. This suggests that, similar to the case of $p \geq q$, the hypercontractive setting may be qualitatively different when $2$ does not lie between $p$ and $q$. - For all $p \geq q$ with $2 \in [q,p]$, we show $\|A\|_{p\rightarrow q}$ is hard to approximate within any factor than $1/(\gamma_{p^*} \cdot \gamma_q)$, where for any $r$, $\gamma_r$ denotes the $r^{th}$ norm of a gaussian, and $p^*$ is the dual norm of $p$.

==> 2_to_p__hardness.tex <==
%%%%%%% Euiwoong's Macros



\begin{document}

\title{$2 \to p$-hardness}

\date{}

\maketitle

\section{Notation}
Currently following BRS15.

\section{Theorem}
We prove the following generalization of Theorem 3.1 of BRS15.
\begin{theorem}
Let $(X_n)_{n \in \NN}$ be a family of finite-dimensional Banach spaces, and $p, \eta, \tau$ be positive numbers such that $1 \leq p < 2$ and $\eta > \tau$. Suppose that for each positive integer $n$ there exists a linear operator $f : \RR^n \to X_n$ with the following properties.
\begin{itemize}
\item For any vector $a \in \RR^n$, we have $\norm{X_n}{f(a)} \leq \ltwonorm{a}$. 
\item For each standard basis vector $e_i$, we have $\norm{X_n}{f(e_i)} \geq \eta$. 
\item For any $\epsilon > 0$, there is a $\delta = \delta(\epsilon)$ such that $\norm{X_n}{f(a)} > (\tau + \epsilon) \ltwonorm{a}$ implies $\lpnorm{4}{a} > \delta \ltwonorm{a}$. 
\end{itemize}
Then, for any $\epsilon' > 0$ there exists a positive integer $n$ such that it is NP-hard to approximate the norm of an explicitly given linear operator $\calf : L_2 \to L_p(X_n)$ to within a factor greater than $(\tau / \eta) + \epsilon'$. 
\label{thm:BRS}
\end{theorem}
\begin{remark}
Their theorem 3.1 is exactly this when $p = 1$ and for $\CC^n$ instead of $\RR^n$, but they explicitly mentioned that the same proof works for $\RR^n$. 
\end{remark}
The reduction and the completeness are identical. 
We prove the following lemma that generalizes Lemma 3.3 of BRS15.
\begin{lemma}
For any $\epsilon > 0$ there exists $\xi, \gamma > 0$ such that $\norm{}{\calf}^p > \tau^p + 4\epsilon^{2 - p}$ then there exists an assignment that satisfies at least $\xi$-fraction of the edges of $G$. 
\end{lemma}
\begin{remark}
Their Lemma 3.3 is exactly this when $p = 1$. 
\end{remark}
The proof is almost the same as the their proof of Lemma 3.3.
Let $\bb \in \calh$ be a vector such that $\Lnorm{2}{\bb} = 1$ and 
\begin{equation}
\E_{v \in V} [\norm{}{f(b_v)}^p] = \Lpnorm{p}{\calf(\bb)}^p \geq \tau^p + 4 \epsilon^{2 - p}. 
\label{eq:soundness}
\end{equation}
Using the third condition in Theorem~\ref{thm:BRS} to obtain $\delta = \delta(\epsilon)$ such that 
$\norm{X_n}{f(a)}^p > (\tau^p + \epsilon) \ltwonorm{a}^p$ implies $\lpnorm{4}{a} > \delta \ltwonorm{a}$,
and consider 
\begin{equation}
V_0 := \{ v \in V : \lpnorm{4}{b_v} > \delta \epsilon \mbox{ and } \ltwonorm{b_v} \leq 1/\epsilon \}.
\label{eq:vzero}
\end{equation}
We give a new proof of the only sub-lemma that concerns the norm of $\calf$. 
\begin{lemma}
[Lemma 3.4 of BRS15]
For $V_0 \subseteq V$ defined as in~\eqref{eq:vzero}, we have $|V_0| \geq \epsilon^2 |V|$. 
\end{lemma}
\begin{proof}
Define the sets
\begin{align*}
V_1 &= \{ v \in V : \lpnorm{4}{b_v} \leq \delta \epsilon \mbox{ and } \ltwonorm{b_v} < \epsilon \}, \\
V_2 &= \{ v \in V : \lpnorm{4}{b_v} \leq \delta \epsilon \mbox{ and } \ltwonorm{b_v} \geq \epsilon \}, \\
V_3 &= \{ v \in V : \ltwonorm{b_v} > 1/\epsilon \}.
\end{align*}
From~\eqref{eq:soundness}, we have
\begin{equation}
\sum_{v \in V_0} \norm{X_n}{f(b_v)}^p +
\sum_{v \in V_1} \norm{X_n}{f(b_v)}^p +
\sum_{v \in V_2} \norm{X_n}{f(b_v)}^p +
\sum_{v \in V_3} \norm{X_n}{f(b_v)}^p \geq (\tau^p + 4 \epsilon^{2 - p}) |V|. 
\label{eq:soundness_sum}
\end{equation}
We bound the four sums on the left side of~\eqref{eq:soundness_sum} individually.
Since (by the first item in Theorem~\ref{thm:BRS}) we have $\norm{X_n}{f(b_v)} \leq \ltwonorm{b_v}$, 
and since $\ltwonorm{b_v} \leq 1/\epsilon$ for every $v \in V_0$, the first sum in~\eqref{eq:soundness_sum} can be bounded by 
\begin{equation}
\sum_{v \in V_0} \norm{X_n}{f(b_v)}^p \leq |V_0| / \epsilon^p.
\label{eq:soundness_zero}
\end{equation}
Similarly, using the definition of $V_1$ the second sum in~\eqref{eq:soundness_sum} is at most $\epsilon^p |V|$. 
Next, from the third property of $f$ in Theorem~\ref{thm:BRS}, for each $v \in V_2$, we have
$\norm{X_n}{f(b_v)}^p \leq (\tau^p + \epsilon) \ltwonorm{b_v}^p$. Therefore, the third sum in~\eqref{eq:soundness_sum} is bounded as 
\begin{align}
\sum_{v \in V_2} \norm{X_n}{f(b_v)}^p 
&\leq (\tau^p + \epsilon) \sum_{v \in V_2} \ltwonorm{b_v}^p    &   \nonumber \\
&= (\tau^p + \epsilon) |V_2| \E_{v \in V_2} [ \ltwonorm{b_v}^p ] &     \nonumber \\
&\leq (\tau^p + \epsilon) |V_2| \E_{v \in V_2} [ \ltwonorm{b_v}^2 ]^{p / 2} && \mbox{(By Jensen using $p < 2$)}    \nonumber \\
&= (\tau^p + \epsilon) |V_2| \bigg( \frac{\sum_{v \in V_2} \ltwonorm{b_v}^2 }{|V_2|} \bigg) ^{p / 2} & \nonumber \\
&\leq (\tau^p + \epsilon) |V_2|^{1 - p / 2} |V|^{p / 2} && (\sum_{v \in V_2} \ltwonorm{b_v}^2 \leq \sum_{v \in V} \ltwonorm{b_v}^2 = |V|) \nonumber \\
&\leq (\tau^p + \epsilon) |V|. &
\end{align}
Finally, the fourth sum in~\eqref{eq:soundness_sum} is bounded by 
\begin{align}
\sum_{v \in V_3} \norm{X_n}{f(b_v)}^p 
&\leq \sum_{v \in V_3} \ltwonorm{b_v}^p    && \mbox{(By the property of $f$)}   \nonumber \\
&= \sum_{v \in V_3} \ltwonorm{b_v}^{p - 2} \ltwonorm{b_v}^2 \nonumber \\
&< \sum_{v \in V_3} \epsilon^{2 - p} \ltwonorm{b_v}^2    && (\ltwonorm{b_v} > 1/\epsilon \mbox{ for } v \in V_3, \mbox{ and } p < 2)  \nonumber \\
&= \epsilon^{2 - p} \sum_{v \in V_3} \ltwonorm{b_v}^2 \leq \epsilon^{2- p} |V|. && 
\end{align}
Combining the above with~\eqref{eq:soundness_sum} yields
\begin{align}
|V_0| 
& \geq \epsilon^{p} \sum_{v \in V_0} \norm{X_n}{f(b_v)}^p  \nonumber \\
& \geq \epsilon^{p} \bigg( (\tau^p + 4 \epsilon^{2 - p}) |V| - \epsilon^p |V| - (\tau^p + \epsilon)|V| - \epsilon^{2-p} |V| \bigg)  \nonumber \\
& \geq \epsilon^{p} \epsilon^{2 - p} |V|  = \epsilon^2 |V|,
\end{align}
where the last inequality uses the fact that $\epsilon^{2- p } \geq \epsilon \geq \epsilon^p$. 
\end{proof}
Equipped with this lemma, the rest of the proof works verbatim as it does not use $\norm{}{\calf}$. 
\end{document}

